Modular Domain Adaptation

Off-the-shelf models are widely used by computational social science researchers to measure properties of text, such as sentiment. However, without access to source data it is difficult to account for domain shift, which represents a threat to validity. Here, we treat domain adaptation as a modular process that involves separate model producers and model consumers, and show how they can independently cooperate to facilitate more accurate measurements of text. We introduce two lightweight techniques for this scenario, and demonstrate that they reliably increase out-of-domain accuracy on four multi-domain text classification datasets when used with linear and contextual embedding models. We conclude with recommendations for model producers and consumers, and release models and replication code to accompany this paper.

==> sections/91_implementation_details.tex <==


\section{Model Details}
\label{appendix:models}

This section formulates a lexicon model and a contextual embedding model with optional usage of numerous techniques we propose. See the next subsection for detailed explanations on each technique.


\subsubsection{Lexicon Model}


We build our lexicon model using logistic regression as the base model, which has the advantage of having learnable parameters in a single linear layer, and is thus interpretable as a weighted lexicon for each class in the multi-class setting. See figure \ref{fig:model-fig-lexicon}, we formulate the base model with our proposed techniques as such:
\begin{equation*}
\begin{split}
    x' &= SN(x) \\
    e &= W_{in} \cdot x' \\
    \hat y &= W_{out} \cdot e \\
    \hat s &= GR(e) \\
    \hat{b_s} &= LR(s) \\
    \hat{b_{c_s}} &= SSB(c_s) \\
    \hat y^* &= \hat y + \hat{b_s} + \hat{b_{c_s}}
\end{split}
\end{equation*}

$x = [x_1, x_2 ... x_{|V|}] \in \mathbf{R}^{|V|}$ is the word features of a single text sample represented by vector of indicator variables $x_v$ whose value is 1 if the word $v$ is present and 0 otherwise; we lowercase all words but do not lemmatize. $s \in \mathbf{R}^{|S|}$ is a vector of one-hot encoding of the source from which this text sample originates. $c_s$ has elements ${c_s}_k = \frac{1}{N_s} \sum_i^{N_s} \mathbf{1} [y^{(i)} = k]$ that describes the likelihood of class $k$ being present in source $s$. 

At training time, we apply a softmax function to $\hat y^*$ and then use categorical cross-entropy loss against the one-hot encoding of the true label of the sample $y$ to optimize for the model. If GR is enabled, we also do the same for $\hat s$ and take the sum of loss. In practice, if it is a multi-label prediction task, a sigmoid activation and a sum of binary cross-entropy for each class can also be used.

Observe that there is no non-linearity between $W_{in}$ and $W_{out}$, and therefore the learned model effectively has a single weight matrix $W_{out} \cdot W_{in} = W \in \mathbf{R}^{K \times |V|}$. After training the model, we can elicit a weighted lexicon by taking the value of $W_{kv}$ to be the association score of word $v$ in class $k$. 


\subsubsection{Contextual Embedding Model}


Transformer models such as RoBERTa \cite{liu2019roberta} have been shown to be powerful language models that achieve high performance in various natural language tasks. Huggingface \cite{wolf2020huggingfaces} is a popular implementation of RoBERTa, with pre-trained weights publicly available. Using a pre-trained RoBERTa base model, we construct the classifier with our proposed technique as seen on figure \ref{fig:model-fig-roberta}:
\begin{equation*}
\begin{split}
    e_{<s>} &= T_{roberta}([\texttt{<s>}, BPE(x)]) \\
    \hat y &= FC(e_{<s>}) \\
    \hat{b_s} &= LR(s) \\
    \hat{b_{c_s}} &= SSB(c_s) \\
    \hat y^* &= \hat y + \hat{b_s} + \hat{b_{c_s}}
\end{split}
\end{equation*}

$BPE$ is the RoBERTa tokenizer that splits the text into sub-word tokens using byte-pair encoding. $T_{roberta}$ is the transformer layers of a pre-trained RoBERTa model. $<s>$ is the special RoBERTa token we prepend to the tokenized text to indicate a classification task, and we take the output embedding of only that token $e_{<s>}$ to be the contextual embedding of the full text. $FC$ is a fully-connected network of any kind; in our experiment, we use a two-layer network with dropout layer and a Tanh activation function between. We similarly apply a softmax function to $\hat y^*$ and then use categorical cross-entropy loss against the one-hot encoding of the true label of the sample $y$ to optimize for the model.
